Automated rapid follow-up of Swift GRBs with AMI-LA

We present 15-GHz follow-up radio observations of eleven Swift gamma-ray burst (GRB) sources, obtained with the Arcminute Microkelvin Imager Large Array (AMI-LA). The initial follow-up observation for each source was made in a fully automated fashion; as a result four observations were initiated within five minutes of the GRB alert timestamp. These observations provide the first millijansky-level constraints on prolonged radio emission from GRBs within the first hour post-burst. While no radio emission within the first six hours after the GRB is detected in this preliminary analysis, radio afterglow is detected from one of the GRBs (GRB120326A) on a timescale of days. The observations were made as part of an ongoing programme to use AMI-LA as a systematic follow-up tool for transients at radio frequencies. In addition to the preliminary results, we explain how we have created an easily extensible automated follow-up system, describing new software tools developed for astronomical transient alert distribution, automatic requesting of target-of-opportunity observations, and robotic control of the observatory.

==> ami_swift_plots.tex <==
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=2cm]{ami_lightcurves/plots/legend}
  \caption[Legend for radio lightcurves]{Legend for radio lightcurves in figures~\ref{fig:GRB120305A}--\ref{fig:GRB120514A}. High-resolution, colour versions of the plots are available online.}
  \label{fig:legend}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120305A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120305A}
  \caption[GRB120305A]{Lightcurves for GRB120305A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120305A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120308A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120308A}
  \caption[GRB120308A]{Lightcurves for GRB120308A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120308A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120311A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120311A}
  \caption[GRB120311A]{Lightcurves for GRB120311A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120311A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120320A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120320A}
  \caption[GRB120320A]{Lightcurves for GRB120320A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120320A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120324A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120324A}
  \caption[GRB120324A]{Lightcurves for GRB120324A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120324A}
\end{center} 
\end{figure}

\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120403A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120403A}
  \caption[GRB120403A]{Lightcurves for GRB120403A. Top: \textit{Swift} BAT lightcurve. 
    No XRT data are available due to Sun observing constraints.
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120403A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120404A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120404A}
  \caption[GRB120404A]{Lightcurves for GRB120404A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120404A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120422A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120422A}
  \caption[GRB120422A]{Lightcurves for GRB120422A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120422A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120514A}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120514A}
  \caption[GRB120514A]{Lightcurves for GRB120514A. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120514A}
\end{center} 
\end{figure}

%NB this file is generated from a template, do not make hand edits!
\begin{figure}%[!p]
\begin{center}  
    \includegraphics[height=5cm]{swift_data/ar_plots/GRB120521C}
    \includegraphics[height=4.5cm]{ami_lightcurves/plots/GRB120521C}
  \caption[GRB120521C]{Lightcurves for GRB120521C. Top: \textit{Swift} BAT/XRT lightcurve. 
    Bottom: Radio lightcurve (See figure~\ref{fig:legend} for legend). 
    Further details in text.}
  \label{fig:GRB120521C}
\end{center} 
\end{figure}


